TAGLETS: A System for Automatic Semi-Supervised Learning with Auxiliary Data

Machine learning practitioners often have access to a spectrum of data: labeled data for the target task (which is often limited), unlabeled data, and auxiliary data, the many available labeled datasets for other tasks. We describe TAGLETS, a system built to study techniques for automatically exploiting all three types of data and creating high-quality, servable classifiers. The key components of TAGLETS are: (1) auxiliary data organized according to a knowledge graph, (2) modules encapsulating different methods for exploiting auxiliary and unlabeled data, and (3) a distillation stage in which the ensembled modules are combined into a servable model. We compare TAGLETS with state-of-the-art transfer learning and semi-supervised learning methods on four image classification tasks. Our study covers a range of settings, varying the amount of labeled data and the semantic relatedness of the auxiliary data to the target task. We find that the intelligent incorporation of auxiliary and unlabeled data into multiple learning techniques enables TAGLETS to match-and most often significantly surpass-these alternatives. TAGLETS is available as an open-source system at github.com/BatsResearch/taglets.

==> tables/accuracy_all.tex <==




\begin{table*}[h]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcccccccccccc}
    \toprule
    Method & Backbone & \multicolumn{3}{c}{OfficeHome-Product} & \multicolumn{3}{c}{OfficeHome-Clipart} & \multicolumn{2}{c}{Grocery Store Dataset} & \multicolumn{3}{c}{Flickr Material Dataset}\\
    \midrule
    & & 1-shot & 5-shot & 20-shot & 1-shot & 5-shot & 20-shot  & 1-shot & 5-shot & 1-shot & 5-shot & 20-shot\\
    \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-10} \cmidrule(lr){11-13}
    Fine-tuning & BiT (ImageNet-21k) & 57.28 $\pm$ 5.20 & 84.41 $\pm$ 1.17 & \textbf{90.67 $\pm$ 1.10} & 30.36 $\pm$ 2.54 & 63.44 $\pm$ 2.10 & \textbf{77.13 $\pm$ 1.34} & 51.32 $\pm$ 3.23 & 85.16 $\pm$ 2.41 & 52.67 $\pm$ 2.35 & 70.07 $\pm$ 1.52 & \textbf{85.40 $\pm$ 0.99}\\
    Fine-tuning (Distilled) & BiT (ImageNet-21k) & 58.21 $\pm$ 4.56 & 85.03 $\pm$ 0.22 & \textbf{92.00 $\pm$ 0.38} & 31.74 $\pm$ 1.96 & 62.92 $\pm$ 1.99 & \textbf{78.26 $\pm$ 0.88} & 52.42 $\pm$ 1.03 & 86.06 $\pm$ 1.81 & 57.53 $\pm$ 10.95 & 73.27 $\pm$ 1.03 & \textbf{86.80 $\pm$ 1.31}\\
    FixMatch & BiT (ImageNet-21k) & 49.03 $\pm$ 2.54 & 83.03 $\pm$ 2.97 & \textbf{92.21 $\pm$ 0.44} & 30.67 $\pm$ 5.44 & 64.77 $\pm$ 1.75 & \textbf{79.95 $\pm$ 2.30} & 48.58 $\pm$ 13.41 & 87.61 $\pm$ 4.82 & 19.07 $\pm$ 31.91 & 60.67 $\pm$ 5.03 & \textbf{84.40 $\pm$ 2.28}\\
    Meta Pseudo Label & BiT (ImageNet-21k) & 59.95 $\pm$ 0.44 & 81.53 $\pm$ 1.01 & \textbf{89.90 $\pm$ 0.88} & 31.74 $\pm$ 2.1 & 62.92 $\pm$ 2.13 & 76.05 $\pm$ 1.72 & 54.51 $\pm$ 6.22 & 84.02 $\pm$ 1.30 & 52.73 $\pm$ 5.82 & 69.80 $\pm$ 2.24 & 79.33 $\pm$ 2.24\\
    TAGLETS & BiT (ImageNet-21k) & \textbf{70.92 $\pm$ 1.67} & \textbf{86.31 $\pm$ 1.01} & \textbf{92.36 $\pm$ 3.18} & \textbf{46.97 $\pm$ 2.46} & \textbf{67.64 $\pm$ 3.34} & \textbf{78.62 $\pm$ 2.76} & \textbf{61.60 $\pm$ 2.90} & \textbf{88.91 $\pm$ 1.07} & \textbf{68.07 $\pm$ 5.76} & \textbf{75.20 $\pm$ 1.72} & \textbf{84.53 $\pm$ 2.29}\\
     \midrule
     TAGLETS prune-level 0 & BiT (ImageNet-21k) & 68.46 $\pm$ 2.13 & 84.92 $\pm$ 0.66 & 92.72 $\pm$ 0.96 & 45.44 $\pm$ 4.05 & 65.69 $\pm$ 2.13 & 78.62 $\pm$ 2.51 & 59.30 $\pm$ 3.88 & 88.69 $\pm$ 3.16 & 67.20 $\pm$ 6.57 & 72.53 $\pm$ 3.49 & 84.13 $\pm$ 1.74\\
     TAGLETS prune-level 1 & BiT (ImageNet-21k) & 67.23 $\pm$ 4.03 & 83.90 $\pm$ 2.46 & 91.95 $\pm$ 0.88 & 41.64 $\pm$ 1.59 & 63.03 $\pm$ 2.71 & 77.38 $\pm$ 1.38 & 52.96 $\pm$ 4.51 & 87.19 $\pm$ 2.81 & 65.07 $\pm$ 4.34 & 73.60 $\pm$ 1.31 & 83.13 $\pm$ 0.29\\
    \midrule
    Fine-tuning & ResNet-50 (ImageNet-1k) & 32.51 $\pm$ 3.83 & 63.44 $\pm$ 7.45 & 81.13 $\pm$ 0.22 & 16.26 $\pm$ 2.87 & 43.49 $\pm$ 0.58 & 68.56 $\pm$ 2.24 & 30.25 $\pm$ 4.08 & 70.60 $\pm$ 3.25 & 28.20 $\pm$ 3.48 & 47.20 $\pm$ 3.94 & 60.47 $\pm$ 8.52\\
    Fine-tuning (Distilled) & ResNet-50 (ImageNet-1k) & 32.72 $\pm$ 3.67 & 66.87 $\pm$ 5.60 & 83.85 $\pm$ 2.68 & 15.85 $\pm$ 0.66 & 44.26 $\pm$ 2.34 & \underline{72.00 $\pm$ 2.32} & 30.64 $\pm$ 4.33 & 74.63 $\pm$ 2.44 & 29.20 $\pm$ 7.32 & 49.80 $\pm$ 3.44 & 66.27 $\pm$ 4.51\\
    FixMatch & ResNet-50 (ImageNet-1k) & 39.28 $\pm$ 3.34 & 72.87 $\pm$ 1.45 & 85.03 $\pm$ 1.81 & 20.51 $\pm$ 0.96 & 49.69 $\pm$ 3.31 & 66.56 $\pm$ 1.23 & 32.14 $\pm$ 4.72 & 70.77 $\pm$ 0.75 & 37.73 $\pm$ 13.97 & 61.00 $\pm$ 6.72 & 74.13 $\pm$ 1.52 \\
    Meta Pseudo Label & ResNet-50 (ImageNet-1k) & 47.38 $\pm$ 2.98 & 76.67 $\pm$ 1.75 & \underline{87.38 $\pm$ 1.75} & 22.77 $\pm$ 3.99 & 57.25 $\pm$ 4.64 & \underline{75.17 $\pm$ 1.22} & 34.68 $\pm$ 3.11 & 75.16 $\pm$ 1.57 & 37.99 $\pm$ 13.52 & \underline{68.00 $\pm$ 3.47} & \underline{77.13 $\pm$ 1.25}\\
    TAGLETS & ResNet-50 (ImageNet-1k) & \underline{67.64 $\pm$ 3.61} & \underline{83.54 $\pm$ 2.89} & \underline{88.77 $\pm$ 2.89} & \underline{43.44 $\pm$ 4.46} & \underline{63.90 $\pm$ 1.17} & \underline{75.54 $\pm$ 4.34} & \underline{51.76 $\pm$ 3.48} & \underline{84.35 $\pm$ 0.92} &  \underline{55.87 $\pm$ 4.05} & \underline{68.27 $\pm$ 2.45} & 74.53 $\pm$ 2.74 \\
    \midrule
    TAGLETS prune-level 0 & ResNet-50 (ImageNet-1k) & \underline{65.33 $\pm$ 1.23} & \underline{81.23 $\pm$ 0.00} & \underline{88.62 $\pm$ 1.38} & \underline{41.49 $\pm$ 1.54} & 62.21 $\pm$ 1.89 & \underline{75.79 $\pm$ 3.11} & 46.32 $\pm$ 5.01 & 81.88 $\pm$ 1.27 & \underline{53.40 $\pm$ 4.42} & \underline{67.60 $\pm$ 3.48} & \underline{74.47 $\pm$ 1.88}\\
    TAGLETS prune-level 1 & ResNet-50 (ImageNet-1k) & 57.28 $\pm$ 1.89 & 76.21 $\pm$ 1.54 & \underline{86.67 $\pm$ 0.58} & 36.87 $\pm$ 2.17 & 55.33 $\pm$ 4.19 & \underline{72.72 $\pm$ 0.96} & 37.68 $\pm$ 6.64 & 75.75 $\pm$ 1.84 & \underline{55.00 $\pm$ 8.18} & \underline{66.00 $\pm$ 5.73} & \underline{72.93 $\pm$ 1.60}\\
    \bottomrule
    \end{tabular}}
    \caption{Accuracy (\%) of \sys and baselines on the four datasets (\texttt{Split 0}) for increasing number of labeled examples (1, 5, and 20 shots), different backbones (ResNet-50 trained on ImageNet-1k and BiT trained on ImageNet-21k) and levels of pruning (no-pruning, 0 and 1). We make bold and underline the best performing models, and all those within their 95\% confidence intervals, carried out using \textbf{BiT} and \underline{ResNet} backbones, respectively. Measurements are repeated for three seeds, and we report the 95\% confidence intervals.}
\label{tab:acc:all}
\end{table*}

==> tables/accuracy_grocery_and_fmd_split1.tex <==
\begin{table*}[ht]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcccccc}
    \toprule
    Method & Backbone & \multicolumn{2}{c}{Grocery Store Dataset} & \multicolumn{3}{c}{Flickr Material Dataset}\\
    \midrule
    & & 1-shot & 5-shot & 1-shot & 5-shot & 20-shot\\
    \cmidrule(lr){3-4} \cmidrule(lr){5-7}
    Fine-tuning & BiT (ImageNet-21k) & 60.52 $\pm$ 4.55 & 84.02 $\pm$ 1.06 & 42.47 $\pm$ 1.88 & 76.27 $\pm$ 3.86 & \textbf{87.40 $\pm$ 0.86}\\
    Fine-tuning (Distilled) & BiT (ImageNet-21k) & 60.56 $\pm$ 5.02 & 85.42 $\pm$ 2.61 & 45.07 $\pm$ 2.45 & \textbf{77.93 $\pm$ 0.29} & \textbf{87.67 $\pm$ 1.15}\\
    FixMatch & BiT (ImageNet-21k) & 48.58 $\pm$ 13.41 & \textbf{87.61 $\pm$ 4.82} & 12.60 $\pm$ 11.19 & 70.73 $\pm$ 10.84 & 86.47 $\pm$ 2.07\\
    Meta Pseudo Label & BiT (ImageNet-21k) & 59.52 $\pm$ 3.96 & 85.58 $\pm$ 0.75 & 44.73 $\pm$ 5.35  & 75.20 $\pm$ 3.44 & 80.73 $\pm$ 2.45\\
    TAGLETS & BiT (ImageNet-21k) & \textbf{66.26 $\pm$ 5.60} & \textbf{87.87 $\pm$ 0.95} & \textbf{60.80 $\pm$ 3.97} &77.60 $\pm$ 4.24 & \textbf{86.67 $\pm$ 1.03}\\
    \midrule
    Fine-tuning & ResNet-50 (ImageNet-1k) & 34.86 $\pm$ 4.11 & 67.23 $\pm$ 0.80 & 25.33 $\pm$ 2.83 & 41.53 $\pm$ 2.91 & 61.93 $\pm$ 3.86\\
    Fine-tuning (Distilled) & ResNet-50 (ImageNet-1k) & 36.31 $\pm$ 1.70 & 72.22 $\pm$ 2.91 & 26.80 $\pm$ 1.31 & 40.80 $\pm$ 6.88 & 64.80 $\pm$ 3.48\\
    FixMatch & ResNet-50 (ImageNet-1k) & 32.69 $\pm$ 1.85 & 71.60 $\pm$ 4.17 & 28.80 $\pm$ 4.24 & 58.80 $\pm$ 4.74 & 75.20 $\pm$ 1.31\\
    Meta Pseudo Label & ResNet-50 (ImageNet-1k) & 38.19 $\pm$ 5.33 & 75.51 $\pm$ 0.47 & 38.44 $\pm$ 10.20 & 65.13 $\pm$ 5.35 & \underline{78.07 $\pm$ 2.50}\\
    TAGLETS & ResNet-50 (ImageNet-1k) & \underline{56.45 $\pm$ 1.90} & \underline{82.43 $\pm$ 1.76} & \underline{51.87 $\pm$ 3.38} & \underline{68.53 $\pm$ 2.24 }& 73.53 $\pm$ 1.43\\
    \midrule
    TAGLETS prune-level 0 & ResNet-50 (ImageNet-1k) & 49.99 $\pm$ 1.85 & 80.24 $\pm$ 2.07 & \underline{48.53 $\pm$ 2.29} & 62.20 $\pm$ 4.74 & 73.00 $\pm$ 2.28\\
    TAGLETS prune-level 1 & ResNet-50 (ImageNet-1k) & 42.91 $\pm$ 9.81 & 73.35 $\pm$ 3.25 & \underline{50.07 $\pm$ 5.80} & \underline{66.67 $\pm$ 3.76} & 72.93 $\pm$ 1.03\\
    \bottomrule
     \end{tabular}}
    \caption{Accuracy (\%) of \sys and baselines on \emph{Grocery Store} and \emph{Flicker Material Datasets} (\texttt{Split 1}) for increasing number of labeled examples (1, 5, and 20 shots), different backbones (ResNet-50 trained on ImageNet-1k and BiT trained on ImageNet-21k) and levels of pruning (no-pruning, 0 and 1). We make bold and underline the best performances, and all those within their 95\% confidence intervals, carried out using \textbf{BiT} and \underline{ResNet} backbones, respectively. Measurements are repeated for three seeds and we report the 95\% confidence intervals.}
\label{tab:acc:gs_and_fms_split1}
\end{table*}

==> tables/accuracy_grocery_and_fmd_split2.tex <==
\begin{table*}[ht]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lcccccc}
    \toprule
    Method & Backbone & \multicolumn{2}{c}{Grocery Store Dataset} & \multicolumn{3}{c}{Flickr Material Dataset}\\
    \midrule
    & & 1-shot & 5-shot & 1-shot & 5-shot & 20-shot\\
    \cmidrule(lr){3-4} \cmidrule(lr){5-7}
    Fine-tuning & BiT (ImageNet-21k) & 60.08 $\pm$ 1.66 & 83.61 $\pm$ 0.71 & 41.07 $\pm$ 6.96 & 69.40 $\pm$ 2.17 & \textbf{85.07 $\pm$ 1.52}\\
    Fine-tuning (Distilled) & BiT (ImageNet-21k) & 62.72 $\pm$ 2.66 & \textbf{84.10 $\pm$ 1.14} & 42.53 $\pm$ 6.21 & 70.93 $\pm$ 2.74 & \textbf{84.53 $\pm$ 1.03}\\
    FixMatch & BiT (ImageNet-21k) & 60.16 $\pm$ 6.51 & \textbf{87.08 $\pm$ 3.30} & 12.13 $\pm$ 8.32 &\textbf{ 72.40 $\pm$ 1.31} & \textbf{83.60 $\pm$ 2.77}\\
    Meta Pseudo Label & BiT (ImageNet-21k) & 62.12 $\pm$ 3.12 & 82.19 $\pm$ 0.21 & 48.86 $\pm$ 8.90 &\textbf{ 74.06 $\pm$ 2.01} & 78.79 $\pm$ 1.31\\
    TAGLETS & BiT (ImageNet-21k) & \textbf{68.26 $\pm$ 3.29} & \textbf{85.88 $\pm$ 0.56} & \textbf{59.60 $\pm$ 9.48} & \textbf{73.47 $\pm$ 2.87} & \textbf{84.27 $\pm$ 1.88}\\
    \midrule
    Fine-tuning & ResNet-50 (ImageNet-1k) & 31.99 $\pm$ 5.14 & 65.78 $\pm$ 4.85 & 28.00 $\pm$ 4.07 & 44.40 $\pm$ 1.72 & 58.80 $\pm$ 5.16\\
    Fine-tuning (Distilled) & ResNet-50 (ImageNet-1k) & 33.17 $\pm$ 2.66 & 69.59 $\pm$ 3.50 & 27.60 $\pm$ 10.57 & 46.07 $\pm$ 7.03 & 62.73 $\pm$ 5.27\\
    FixMatch & ResNet-50 (ImageNet-1k) & 37.64 $\pm$ 1.50 & 68.10 $\pm$ 2.86 & 35.80 $\pm$ 12.41 & 57.40 $\pm$ 5.23 & 69.73 $\pm$ 2.55\\
    Meta Pseudo Label & ResNet-50 (ImageNet-1k) & 39.46 $\pm$ 0.97 & 70.03 $\pm$ 1.35 & 38.66 $\pm$ 2.57 & \underline{65.66 $\pm$ 5.31} & \underline{75.46 $\pm$ 2.99}\\
    TAGLETS & ResNet-50 (ImageNet-1k) & \underline{57.45 $\pm$ 5.66} & \underline{81.57 $\pm$ 1.04} & \underline{53.13 $\pm$ 6.29} & \underline{65.87 $\pm$ 1.74} & \underline{72.80 $\pm$ 2.28}\\
    \midrule
    TAGLETS prune-level 0 & ResNet-50 (ImageNet-1k) & \underline{55.36 $\pm$ 6.00} & 79.38 $\pm$ 2.47 & \underline{51.67 $\pm$ 3.31} & \underline{64.53 $\pm$ 2.99} & 71.80 $\pm$ 3.48\\
    TAGLETS prune-level 1 & ResNet-50 (ImageNet-1k) & 47.03 $\pm$ 8.44 & 74.98 $\pm$ 1.36 & 46.00 $\pm$ 15.30 & 62.00 $\pm$ 7.81 & 69.93 $\pm$ 2.24\\
    \bottomrule
     \end{tabular}}
    \caption{Accuracy (\%) of \sys and baselines on \emph{Grocery Store} and \emph{Flicker Material Datasets} (\texttt{Split 2}) for increasing number of labeled examples (1, 5, and 20 shots), different backbones (ResNet-50 trained on ImageNet-1k and BiT trained on ImageNet-21k) and levels of pruning (no-pruning, 0 and 1). We make bold and underline the best performances, and all those within their 95\% confidence intervals, carried out using \textbf{BiT} and \underline{ResNet} backbones, respectively. Measurements are repeated for three seeds and we report the 95\% confidence intervals.}
\label{tab:acc:gs_and_fms_split2}
\end{table*}

==> tables/accuracy_officehome_split1.tex <==
\begin{table*}[t]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lccccccc}
    \toprule
    Method & Backbone & \multicolumn{3}{c}{OfficeHome-Product} & \multicolumn{3}{c}{OfficeHome-Clipart}\\
    \midrule
    & & 1-shot & 5-shot & 20-shot & 1-shot & 5-shot & 20-shot\\
    \cmidrule(lr){3-5} \cmidrule(lr){6-8}
    Fine-tuning & BiT (ImageNet-21k) & 62.56 $\pm$ 2.10 & 84.72 $\pm$ 0.88 & 91.85 $\pm$ 0.38 & 31.85 $\pm$ 4.63 & 65.95 $\pm$ 0.58 & \textbf{80.67 $\pm$ 0.58}\\
    Fine-tuning (Distilled) & BiT (ImageNet-21k) & 62.56 $\pm$ 2.54 & \textbf{85.74 $\pm$ 0.58} & \textbf{92.51 $\pm$ 0.44} & 31.18 $\pm$ 2.46 & 65.44 $\pm$ 0.96 & 78.51 $\pm$ 1.89\\
    FixMatch & BiT (ImageNet-21k) & 56.87 $\pm$ 3.11 & 83.95 $\pm$ 0.96 & 91.64 $\pm$ 1.17 & 28.87 $\pm$ 9.40 & 64.56 $\pm$ 0.58 & 81.59 $\pm$ 1.23\\
    Meta Pseudo Label & BiT (ImageNet-21k) & 61.28 $\pm$ 1.12 & 80.97 $\pm$ 2.60 & 90.77 $\pm$ 1.38 & 31.64 $\pm$ 0.96 & 62.67 $\pm$ 1.72 & 76.15 $\pm$ 1.01\\
    TAGLETS & BiT (ImageNet-21k) &\textbf{ 74.67 $\pm$ 1.45} & \textbf{85.85 $\pm$ 0.66} & 91.95 $\pm$ 0.88 & \textbf{43.64 $\pm$ 5.52} & \textbf{68.05 $\pm$ 1.45} & \textbf{80.41 $\pm$ 3.67}\\
    \midrule
    Fine-tuning & ResNet-50 (ImageNet-1k) & 34.72 $\pm$ 1.10 & 64.97 $\pm$ 0.88 & 84.41 $\pm$ 2.49 & 17.03 $\pm$ 1.89 & 43.85 $\pm$ 3.27 & 69.64 $\pm$ 3.11\\
    Fine-tuning (Distilled) & ResNet-50 (ImageNet-1k) & 35.95 $\pm$ 2.46 & 65.44 $\pm$ 3.85 & 85.79 $\pm$ 0.58 & 16.72 $\pm$ 1.81 & 45.13 $\pm$ 2.49 & 70.92 $\pm$ 2.13\\
    FixMatch & ResNet-50 (ImageNet-1k) & 43.74 $\pm$ 0.80 & 74.31 $\pm$ 1.67 & 85.90 $\pm$ 0.58 & 22.51 $\pm$ 1.17 & 51.38 $\pm$ 3.03 & 67.03 $\pm$ 0.22\\
    Meta Pseudo Label & ResNet-50 (ImageNet-1k) & 51.69 $\pm$ 2.89 & 76.76 $\pm$ 1.38 & 89.75 $\pm$ 0.88 & 23.48 $\pm$ 1.59 & 56.10 $\pm$ 3.18 & \underline{75.40 $\pm$ 1.96}\\
    TAGLETS & ResNet-50 (ImageNet-1k) & \underline{70.92 $\pm$ 3.13} & \underline{82.67 $\pm$ 1.10} & \underline{90.72 $\pm$ 0.96} & \underline{43.28 $\pm$ 0.96} & \underline{64.77 $\pm$ 2.51} & \underline{75.64 $\pm$ 2.68}\\
    \midrule
    TAGLETS prune-level 0 & ResNet-50 (ImageNet-1k) & \underline{68.87 $\pm$ 2.46} & \underline{81.59 $\pm$ 0.58} & \underline{90.51 $\pm$ 1.81} & \underline{42.82 $\pm$ 1.45} & 60.10 $\pm$ 2.10 & \underline{76.05 $\pm$ 2.17}\\
    TAGLETS prune-level 1 & ResNet-50 (ImageNet-1k) & 64.00 $\pm$ 3.40 & 77.59 $\pm$ 1.23 & 88.67 $\pm$ 0.80 & 37.69 $\pm$ 2.29 & 53.23 $\pm$ 2.39 & \underline{74.00 $\pm$ 1.75}\\
    \bottomrule
    \end{tabular}}
    \caption{Accuracy (\%) of \sys and baselines on \emph{OfficeHome Product} and \emph{Clipart} (\texttt{Split 1}) for increasing number of labeled examples (1, 5, and 20 shots), different backbones (ResNet-50 trained on ImageNet-1k and BiT trained on ImageNet-21k) and levels of pruning (no-pruning, 0 and 1). We make bold and underline the best performances, and all those within their 95\% confidence intervals, carried out using \textbf{BiT} and \underline{ResNet} backbones, respectively. Measurements are repeated for three seeds and we report the 95\% confidence intervals.}
\label{tab:acc:officehome_split1}
\end{table*}

==> tables/accuracy_officehome_split2.tex <==
\begin{table*}[h]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lccccccc}
    \toprule
    Method & Backbone & \multicolumn{3}{c}{OfficeHome-Product} & \multicolumn{3}{c}{OfficeHome-Clipart}\\
    \midrule
    & & 1-shot & 5-shot & 20-shot & 1-shot & 5-shot & 20-shot\\
    \cmidrule(lr){3-5} \cmidrule(lr){6-8}
    Fine-tuning & BiT (ImageNet-21k) & 57.49 $\pm$ 1.54 & \textbf{82.51 $\pm$ 1.23} & \textbf{90.56 $\pm$ 0.58} & 32.87 $\pm$ 3.43 & 62.87 $\pm$ 1.10 & \textbf{78.15 $\pm$ 1.32}\\
    Fine-tuning (Distilled) & BiT (ImageNet-21k) & 56.62 $\pm$ 3.99 & \textbf{82.77 $\pm$ 1.75} & \textbf{90.77 $\pm$ 0.66} & 32.92 $\pm$ 5.88 & 62.87 $\pm$ 2.10 & \textbf{78.10 $\pm$ 0.44}\\
    FixMatch & BiT (ImageNet-21k) & 48.15 $\pm$ 1.91 & \textbf{82.41 $\pm$ 1.81} & \textbf{90.46 $\pm$ 0.76} & 9.59 $\pm$ 6.09 & 63.23 $\pm$ 2.65 & \textbf{79.23 $\pm$ 1.38}\\
    Meta Pseudo Label & BiT (ImageNet-21k) & 57.79 $\pm$ 0.58 & 78.61 $\pm$ 1.52 & 88.21 $\pm$ 0.58 & 26.46 $\pm$ 3.90 & 54.31 $\pm$ 2.12 & 75.12 $\pm$ 0.79\\
    TAGLETS & BiT (ImageNet-21k) & \textbf{70.00 $\pm$ 0.76} & \textbf{84.67 $\pm$ 2.30} & \textbf{90.56 $\pm$ 1.72} & \textbf{45.79 $\pm$ 4.19} & \textbf{66.62 $\pm$ 2.13} & \textbf{79.08 $\pm$ 1.32}\\
    \midrule 
    Fine-tuning & ResNet-50 (ImageNet-1k) & 34.36 $\pm$ 3.45 & 63.54 $\pm$ 3.50 & 82.10 $\pm$ 0.96 & 18.92 $\pm$ 1.99 & 41.69 $\pm$ 2.39 & 70.72 $\pm$ 3.55\\
    Fine-tuning (Distilled) & ResNet-50 (ImageNet-1k) & 35.49 $\pm$ 3.83 & 65.90 $\pm$ 3.25 & 84.62 $\pm$ 0.66 & 20.26 $\pm$ 0.44 & 43.85 $\pm$ 4.63 & 72.10 $\pm$ 2.97\\
    FixMatch & ResNet-50 (ImageNet-1k) & 43.38 $\pm$ 3.65 & 72.15 $\pm$ 0.76 & 84.56 $\pm$ 2.10 & 24.05 $\pm$ 1.81 & 49.38 $\pm$ 3.40 & 69.85 $\pm$ 2.39\\
    Meta Pseudo Label & ResNet-50 (ImageNet-1k) & 50.87 $\pm$ 2.10 & 74.87 $\pm$ 2.76 & 88.20 $\pm$ 1.45 & 21.28 $\pm$ 1.22 & 44.41 $\pm$ 1.45 & 70.41 $\pm$ 2.10\\
    TAGLETS & ResNet-50 (ImageNet-1k) & \underline{67.54 $\pm$ 0.00} & \underline{84.62 $\pm$ 1.38} & \underline{89.90 $\pm$ 1.23} & \underline{43.95 $\pm$ 2.10} & \underline{63.18 $\pm$ 1.45} & \underline{78.31 $\pm$ 3.03}\\
    \midrule
    TAGLETS prune-level 0 & ResNet-50 (ImageNet-1k) & 65.33 $\pm$ 0.58 & 82.67 $\pm$ 1.92 & \underline{89.64 $\pm$ 0.22} & \underline{43.59 $\pm$ 1.96} & 59.33 $\pm$ 1.10 & \underline{77.18 $\pm$ 2.54}\\
    TAGLETS prune-level 1 & ResNet-50 (ImageNet-1k) & 60.56 $\pm$ 1.59 & 78.00 $\pm$ 1.53 & \underline{88.82 $\pm$ 0.80} & 39.59 $\pm$ 3.45 & 55.08 $\pm$ 1.99 & \underline{75.49 $\pm$ 1.17}\\
    \bottomrule
    \end{tabular}}
    \caption{Accuracy (\%) of \sys and baselines on \emph{OfficeHome Product} and \emph{Clipart} (\texttt{Split 2}) for increasing number of labeled examples (1, 5, and 20 shots), different backbones (ResNet-50 trained on ImageNet-1k and BiT trained on ImageNet-21k) and levels of pruning (no-pruning, 0 and 1). We make bold and underline the best performances, and all those within their 95\% confidence intervals, carried out using \textbf{BiT} and \underline{ResNet} backbones, respectively. Measurements are repeated for three seeds and we report the 95\% confidence intervals.}
\label{tab:acc:officehome_split2}
\end{table*}

==> tables/before_after_end.tex <==
\begin{table*}[h]
\begin{tabular}{|c|c|c|c|}
\hline
Method                              & Places365-x labels & Dataset 2-x labels  & Dataset 3-x labels \\ \hline
Taglets w/o end model prune-level 2 & xx.xx +/- x.xx     & xx.xx +/- x.xx      & xx.xx +/- x.xx      \\ \hline
Taglets w/o end model prune-level 1 & xx.xx +/- x.xx     & xx.xx +/- x.xx      & xx.xx +/- x.xx\\ \hline
Taglets w/o end model prune-level 0 & xx.xx +/- x.xx     & xx.xx +/- x.xx      & xx.xx +/- x.xx\\ \hline
Taglets prune-level 2               & xx.xx +/- x.xx     & xx.xx +/- x.xx      & xx.xx +/- x.xx\\ \hline
Taglets prune-level 1               & xx.xx +/- x.xx     & xx.xx +/- x.xx      & xx.xx +/- x.xx\\ \hline
Taglets prune-level 0               & xx.xx +/- x.xx     & xx.xx +/- x.xx      & xx.xx +/- x.xx\\ \hline
\end{tabular}
\caption{Accuracy before EndModule vs. after EndModule}
\label{tab:acc:endmodel}
\end{table*}

==> tables/labelmodels.tex <==
% \begin{table}[h]
% \caption{Classification accuracies for naive Bayes and flexible
% Bayes on various data sets.}
% \label{sample-table}
% \vskip 0.15in
% \begin{center}
% \begin{small}
% \begin{sc}
% \begin{tabular}{lcccr}
% \toprule
% Data set & Naive & Flexible & Better? \\
% \midrule
% Breast    & 95.9$\pm$ 0.2& 96.7$\pm$ 0.2& $\surd$ \\
% Cleveland & 83.3$\pm$ 0.6& 80.0$\pm$ 0.6& $\times$\\
% Glass2    & 61.9$\pm$ 1.4& 83.8$\pm$ 0.7& $\surd$ \\
% Credit    & 74.8$\pm$ 0.5& 78.3$\pm$ 0.6&         \\
% Horse     & 73.3$\pm$ 0.9& 69.7$\pm$ 1.0& $\times$\\
% Meta      & 67.1$\pm$ 0.6& 76.5$\pm$ 0.5& $\surd$ \\
% Pima      & 75.1$\pm$ 0.6& 73.9$\pm$ 0.5&         \\
% Vehicle   & 44.9$\pm$ 0.6& 61.5$\pm$ 0.4& $\surd$ \\
% \bottomrule
% \end{tabular}
% \end{sc}
% \end{small}
% \end{center}
% \vskip -0.1in
% \end{table}



\begin{table*}[h]
\begin{tabular}{|c|c|c|}
\hline
LabelModel                  & CIFAR-100-x labels & ImageNet1k-x labels \\ \hline
Majority vote               & xx.xx +/- x.xx     & xx.xx +/- x.xx      \\ \hline
NaiveBayes                  & xx.xx +/- x.xx     & xx.xx +/- x.xx      \\ \hline
HMM                         & xx.xx +/- x.xx     & xx.xx +/- x.xx      \\ \hline
Dylan \& Alessio labelmodel & xx.xx +/- x.xx     & xx.xx +/- x.xx      \\ \hline
\end{tabular}
\caption{Compare LabelModels}
\label{tab:acc:labelmod}
\end{table*}

==> tables/single_modules_ablation.tex <==
\begin{table*}[h]
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{} & \multicolumn{8}{c|}{Places365}                                                                                                       \\ \hline
Method                 & Checkpoint 1   & Checkpoint 2   & Checkpoint 3   & Checkpoint 4   & Checkpoint 5   & Checkpoint 6   & Checkpoint 7   & Checkpoint 8   \\ \hline
Module 1             & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
Module 2             & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
Module 3             & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
Module 1 w Random SCADS            & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
Module 1 w partial SCADS               & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
Module 1 w SCADS               & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
Random Transfer module         & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
Transfer module with prune-level 2         & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
Transfer module with prune-level 1         & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
Transfer module with prune-level 0         & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
Random Multi-task module        & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
Multi-task module with prune-level 2         & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
Multi-task module with prune-level 1         & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
Multi-task module with prune-level 0         & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline \hline
SOTA SSL 1             & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
SOTA SSL 2             & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
SOTA SSL 3             & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
Random FixMatch module         & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
FixMatch module with prune-level 2         & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
FixMatch module with prune-level 1         & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
FixMatch module with prune-level 0         & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
\end{tabular}
\caption{Accuracy of single modules against their corresponding state-of-the-arts}
\label{tab:acc:imagenet}
\end{table*}


==> tables/single_modules_ablation2.tex <==
\begin{table*}[h]
\centering
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\multicolumn{1}{|l|}{} & \multicolumn{6}{c|}{Places365}                                                                                                       \\ \hline
Method                 & 1-shot   & 5-shot   & 20-shot   & 50-shot   & 100-shot   & 500-shot   \\ \hline
TransferModule prune-level 0  & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
MultiTaskModule prune-level 0  & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
ZSLKGModule prune-level 0  & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
FixMatchModule prune-level 0  & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
DANNModule prune-level 0  & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
Taglets prune-level 0  & xx.xx +/- x.xx & xx.xx +/-s x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
TransferModule prune-level 1  & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
MultiTaskModule prune-level 1  & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
ZSLKGModule prune-level 1  & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
FixMatchModule prune-level 1  & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
DANNModule prune-level 1  & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
Taglets prune-level 1  & xx.xx +/- x.xx & xx.xx +/-s x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
TransferModule prune-level 2  & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
MultiTaskModule prune-level 2  & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
ZSLKGModule prune-level 2  & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
FixMatchModule prune-level 2  & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
DANNModule prune-level 2  & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
Taglets prune-level 2  & xx.xx +/- x.xx & xx.xx +/-s x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx & xx.xx +/- x.xx \\ \hline
\end{tabular}
\caption{Places365: \sys accuracy for increasing number of labels compared with relevant transfer learning methods and semi-supervised SOTA}
\label{tab:acc:ablation}
\end{table*}


==> tables/single_modules_few_shots.tex <==
\begin{table*}[h]
\begin{tabular}{|c|c|c|c|c|}
\hline
Method                               & miniImageNet          & TieredImageNet        & CIFAR-FS              & FC-100                \\ \hline
SOTA Few-shot 1                      & xx.xx +/- x.xx        & xx.xx +/- x.xx        & xx.xx +/- x.xx        & xx.xx +/- x.xx        \\ \hline
SOTA Few-shot 2                      & xx.xx +/- x.xx        & xx.xx +/- x.xx        & xx.xx +/- x.xx        & xx.xx +/- x.xx        \\ \hline
SOTA Few-shot 3                      & xx.xx +/- x.xx        & xx.xx +/- x.xx        & xx.xx +/- x.xx        & xx.xx +/- x.xx        \\ \hline
Random Multi-task module             & xx.xx +/- x.xx        & xx.xx +/- x.xx        & xx.xx +/- x.xx        & xx.xx +/- x.xx        \\ \hline
Multi-task module with prune-level 2 & xx.xx +/- x.xx        & xx.xx +/- x.xx        & xx.xx +/- x.xx        & xx.xx +/- x.xx        \\ \hline
Multi-task module with prune-level 1 & xx.xx +/- x.xx        & xx.xx +/- x.xx        & xx.xx +/- x.xx        & xx.xx +/- x.xx        \\ \hline
Multi-task module with prune-level 0 & xx.xx +/- x.xx        & xx.xx +/- x.xx        & xx.xx +/- x.xx        & xx.xx +/- x.xx        \\ \hline
Transfer module with prune-level 2 & xx.xx +/- x.xx        & xx.xx +/- x.xx        & xx.xx +/- x.xx        & xx.xx +/- x.xx        \\ \hline
Transfer module with prune-level 1 & xx.xx +/- x.xx        & xx.xx +/- x.xx        & xx.xx +/- x.xx        & xx.xx +/- x.xx        \\ \hline
Transfer module with prune-level 0 & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
\end{tabular}
\caption{Comparison of few-shot SOTA and related modules on TAGLETS}
\label{tab:fewshot:modules}
\end{table*}


==> tables/single_modules_semi.tex <==
\begin{table*}[h]
\begin{tabular}{|c|c|c|c|c|}
\hline
Method                             & ImageNet1k-1\% & ImageNet1k-10\% & CIFAR-100-400 labels & CIFAR-100-2500 labels \\ \hline
SOTA SSL 1                         & xx.xx +/- x.xx & xx.xx +/- x.xx  & xx.xx +/- x.xx       & xx.xx +/- x.xx        \\ \hline
SOTA SSL 2                         & xx.xx +/- x.xx & xx.xx +/- x.xx  & xx.xx +/- x.xx       & xx.xx +/- x.xx        \\ \hline
SOTA SSL 3                         & xx.xx +/- x.xx & xx.xx +/- x.xx  & xx.xx +/- x.xx       & xx.xx +/- x.xx        \\ \hline
Random FixMatch module             & xx.xx +/- x.xx & xx.xx +/- x.xx  & xx.xx +/- x.xx       & xx.xx +/- x.xx        \\ \hline
FixMatch module with prune-level 2 & -              & -               & xx.xx +/- x.xx       & xx.xx +/- x.xx        \\ \hline
FixMatch module with prune-level 1 & -              & -               & xx.xx +/- x.xx       & xx.xx +/- x.xx        \\ \hline
FixMatch module with prune-level 0 & xx.xx +/- x.xx & xx.xx +/- x.xx  & xx.xx +/- x.xx       & xx.xx +/- x.xx        \\ \hline
\end{tabular}
\caption{Comparison of semi-supervised SOTA and related modules on TAGLETS}
\label{tab:semi:modules}
\end{table*}

==> tables/split_1_and_2_v2.tex <==
\begin{table*}[t]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lccccccc}
    \toprule
    
    Method & Backbone & \multicolumn{3}{c}{OfficeHome-Product} & \multicolumn{3}{c}{OfficeHome-Clipart}\\
    \midrule
    %\textbf{\texttt{Split 1}} & &  &  &  &  &  & \\
    %\midrule
    \textbf{\texttt{Split 1}} &  & 1-shot & 5-shot & 20-shot & 1-shot & 5-shot & 20-shot\\
    \midrule
    %\cmidrule(lr){3-5} \cmidrule(lr){6-8}
    Fine-tuning & BiT (ImageNet-21k) & 62.56 $\pm$ 2.10 & 84.72 $\pm$ 0.88 & 91.85 $\pm$ 0.38 & 31.85 $\pm$ 4.63 & 65.95 $\pm$ 0.58 & \textbf{80.67 $\pm$ 0.58}\\
    Fine-tuning (Distilled) & BiT (ImageNet-21k) & 62.56 $\pm$ 2.54 & \textbf{85.74 $\pm$ 0.58} & \textbf{92.51 $\pm$ 0.44} & 31.18 $\pm$ 2.46 & 65.44 $\pm$ 0.96 & 78.51 $\pm$ 1.89\\
    FixMatch & BiT (ImageNet-21k) & 56.87 $\pm$ 3.11 & 83.95 $\pm$ 0.96 & 91.64 $\pm$ 1.17 & 28.87 $\pm$ 9.40 & 64.56 $\pm$ 0.58 & 81.59 $\pm$ 1.23\\
    Meta Pseudo Label & BiT (ImageNet-21k) & 61.28 $\pm$ 1.12 & 80.97 $\pm$ 2.60 & 90.77 $\pm$ 1.38 & 31.64 $\pm$ 0.96 & 62.67 $\pm$ 1.72 & 76.15 $\pm$ 1.01\\
    TAGLETS & BiT (ImageNet-21k) &\textbf{ 74.67 $\pm$ 1.45} & \textbf{85.85 $\pm$ 0.66} & 91.95 $\pm$ 0.88 & \textbf{43.64 $\pm$ 5.52} & \textbf{68.05 $\pm$ 1.45} & \textbf{80.41 $\pm$ 3.67}\\
    \midrule
    Fine-tuning & ResNet-50 (ImageNet-1k) & 34.72 $\pm$ 1.10 & 64.97 $\pm$ 0.88 & 84.41 $\pm$ 2.49 & 17.03 $\pm$ 1.89 & 43.85 $\pm$ 3.27 & 69.64 $\pm$ 3.11\\
    Fine-tuning (Distilled) & ResNet-50 (ImageNet-1k) & 35.95 $\pm$ 2.46 & 65.44 $\pm$ 3.85 & 85.79 $\pm$ 0.58 & 16.72 $\pm$ 1.81 & 45.13 $\pm$ 2.49 & 70.92 $\pm$ 2.13\\
    FixMatch & ResNet-50 (ImageNet-1k) & 43.74 $\pm$ 0.80 & 74.31 $\pm$ 1.67 & 85.90 $\pm$ 0.58 & 22.51 $\pm$ 1.17 & 51.38 $\pm$ 3.03 & 67.03 $\pm$ 0.22\\
    Meta Pseudo Label & ResNet-50 (ImageNet-1k) & 51.69 $\pm$ 2.89 & 76.76 $\pm$ 1.38 & 89.75 $\pm$ 0.88 & 23.48 $\pm$ 1.59 & 56.10 $\pm$ 3.18 & \underline{75.40 $\pm$ 1.96}\\
    TAGLETS & ResNet-50 (ImageNet-1k) & \underline{70.92 $\pm$ 3.13} & \underline{82.67 $\pm$ 1.10} & \underline{90.72 $\pm$ 0.96} & \underline{43.28 $\pm$ 0.96} & \underline{64.77 $\pm$ 2.51} & \underline{75.64 $\pm$ 2.68}\\
    \midrule
    TAGLETS prune-level 0 & ResNet-50 (ImageNet-1k) & \underline{68.87 $\pm$ 2.46} & \underline{81.59 $\pm$ 0.58} & \underline{90.51 $\pm$ 1.81} & \underline{42.82 $\pm$ 1.45} & 60.10 $\pm$ 2.10 & \underline{76.05 $\pm$ 2.17}\\
    TAGLETS prune-level 1 & ResNet-50 (ImageNet-1k) & 64.00 $\pm$ 3.40 & 77.59 $\pm$ 1.23 & 88.67 $\pm$ 0.80 & 37.69 $\pm$ 2.29 & 53.23 $\pm$ 2.39 & \underline{74.00 $\pm$ 1.75}\\
    %\cmidrule(lr){3-5} \cmidrule(lr){6-8}
    \midrule
    \midrule
    \textbf{\textbf{\texttt{Split 2}}} & & 1-shot & 5-shot & 20-shot & 1-shot & 5-shot & 20-shot \\
    \midrule
    Fine-tuning & BiT (ImageNet-21k) & 57.49 $\pm$ 1.54 & \textbf{82.51 $\pm$ 1.23} & \textbf{90.56 $\pm$ 0.58} & 32.87 $\pm$ 3.43 & 62.87 $\pm$ 1.10 & \textbf{78.15 $\pm$ 1.32}\\
    Fine-tuning (Distilled) & BiT (ImageNet-21k) & 56.62 $\pm$ 3.99 & \textbf{82.77 $\pm$ 1.75} & \textbf{90.77 $\pm$ 0.66} & 32.92 $\pm$ 5.88 & 62.87 $\pm$ 2.10 & \textbf{78.10 $\pm$ 0.44}\\
    FixMatch & BiT (ImageNet-21k) & 48.15 $\pm$ 1.91 & \textbf{82.41 $\pm$ 1.81} & \textbf{90.46 $\pm$ 0.76} & 9.59 $\pm$ 6.09 & 63.23 $\pm$ 2.65 & \textbf{79.23 $\pm$ 1.38}\\
    Meta Pseudo Label & BiT (ImageNet-21k) & 57.79 $\pm$ 0.58 & 78.61 $\pm$ 1.52 & 88.21 $\pm$ 0.58 & 26.46 $\pm$ 3.90 & 54.31 $\pm$ 2.12 & 75.12 $\pm$ 0.79\\
    TAGLETS & BiT (ImageNet-21k) & \textbf{70.00 $\pm$ 0.76} & \textbf{84.67 $\pm$ 2.30} & \textbf{90.56 $\pm$ 1.72} & \textbf{45.79 $\pm$ 4.19} & \textbf{66.62 $\pm$ 2.13} & \textbf{79.08 $\pm$ 1.32}\\
    \midrule 
    Fine-tuning & ResNet-50 (ImageNet-1k) & 34.36 $\pm$ 3.45 & 63.54 $\pm$ 3.50 & 82.10 $\pm$ 0.96 & 18.92 $\pm$ 1.99 & 41.69 $\pm$ 2.39 & 70.72 $\pm$ 3.55\\
    Fine-tuning (Distilled) & ResNet-50 (ImageNet-1k) & 35.49 $\pm$ 3.83 & 65.90 $\pm$ 3.25 & 84.62 $\pm$ 0.66 & 20.26 $\pm$ 0.44 & 43.85 $\pm$ 4.63 & 72.10 $\pm$ 2.97\\
    FixMatch & ResNet-50 (ImageNet-1k) & 43.38 $\pm$ 3.65 & 72.15 $\pm$ 0.76 & 84.56 $\pm$ 2.10 & 24.05 $\pm$ 1.81 & 49.38 $\pm$ 3.40 & 69.85 $\pm$ 2.39\\
    Meta Pseudo Label & ResNet-50 (ImageNet-1k) & 50.87 $\pm$ 2.10 & 74.87 $\pm$ 2.76 & 88.20 $\pm$ 1.45 & 21.28 $\pm$ 1.22 & 44.41 $\pm$ 1.45 & 70.41 $\pm$ 2.10\\
    TAGLETS & ResNet-50 (ImageNet-1k) & \underline{67.54 $\pm$ 0.00} & \underline{84.62 $\pm$ 1.38} & \underline{89.90 $\pm$ 1.23} & \underline{43.95 $\pm$ 2.10} & \underline{63.18 $\pm$ 1.45} & \underline{78.31 $\pm$ 3.03}\\
    \midrule
    TAGLETS prune-level 0 & ResNet-50 (ImageNet-1k) & 65.33 $\pm$ 0.58 & 82.67 $\pm$ 1.92 & \underline{89.64 $\pm$ 0.22} & \underline{43.59 $\pm$ 1.96} & 59.33 $\pm$ 1.10 & \underline{77.18 $\pm$ 2.54}\\
    TAGLETS prune-level 1 & ResNet-50 (ImageNet-1k) & 60.56 $\pm$ 1.59 & 78.00 $\pm$ 1.53 & \underline{88.82 $\pm$ 0.80} & 39.59 $\pm$ 3.45 & 55.08 $\pm$ 1.99 & \underline{75.49 $\pm$ 1.17}\\
    \bottomrule
    \end{tabular}}
    \caption{Accuracy (\%) of \sys and baselines on \emph{OfficeHome Product} and \emph{Clipart} (\texttt{Split 1 and 2}) for increasing number of labeled examples (1, 5, and 20 shots), different backbones (ResNet-50 trained on ImageNet-1k and BiT trained on ImageNet-21k) and levels of pruning (no-pruning, 0 and 1). We make bold and underline the best performances, and all those within their 95\% confidence intervals, carried out using \textbf{BiT} and \underline{ResNet} backbones, respectively. Measurements are repeated for three seeds and we report the 95\% confidence intervals.}
\label{tab:acc:officehome_split1}
\end{table*}
